Polygon-free: Unconstrained Scene Text Detection with Box Annotations

Although a polygon is a more accurate representation than an upright bounding box for text detection, the annotations of polygons are extremely expensive and challenging. Unlike existing works that employ fully-supervised training with polygon annotations, this study proposes an unconstrained text detection system termed Polygon-free (PF), in which most existing polygon-based text detectors (e.g., PSENet [33],DB [16]) are trained with only upright bounding box annotations. Our core idea is to transfer knowledge from synthetic data to real data to enhance the supervision information of upright bounding boxes. This is made possible with a simple segmentation network, namely Skeleton Attention Segmentation Network (SASN), that includes three vital components (i.e., channel attention, spatial attention and skeleton attention map) and one soft cross-entropy loss. Experiments demonstrate that the proposed Polygonfree system can combine general detectors (e.g., EAST, PSENet, DB) to yield surprisingly high-quality pixel-level results with only upright bounding box annotations on a variety of datasets (e.g., ICDAR2019-Art, TotalText, ICDAR2015). For example, without using polygon annotations, PSENet achieves an 80.5% F-score on TotalText [3] (vs. 80.9% of fully supervised counterpart), 31.1% better than training directly with upright bounding box annotations, and saves 80%+ labeling costs. We hope that PF can provide a new perspective for text detection to reduce the labeling costs. The code can be found at https://github.com/weijiawu/Unconstrained-Text-Detection-with-Box-Supervisionand-Dynamic-Self-Training.

==> tables/table2.tex <==
\begin{subtable}[t]{3.2in}
	\centering
% 	\def\x{{$\footnotesize \times$}}
    \setlength{\tabcolsep}{1.3mm}
	\footnotesize
    \begin{tabular}{l|c|c|c|c}
    \whline
	\multirow{2}*{Synthetic Data} & \multirow{2}*{Size}  &\multicolumn{3}{c}{Evaluation on Total-Text/\%}\cr\cline{3-5}  
	~ & ~ & Precision & Recall & F-score \cr\shline \hline
	\hline
    SynthText    & 50k  & 78.3 & 73.5 & 75.9  \\
    SynthText  & 500k  & 80.4 & 74.0 & 77.1  \\
    SynthText  & 1m  & 79.7 & 74.0 & 76.7  \\
    \hline
    Curved SynthText  & 50k  & 80.8 & 75.0 & 77.8  \\
    Curved SynthText  & 500k  & \textbf{81.7} & \textbf{75.6} & \textbf{78.5}  \\
    Curved SynthText  & 1m  & 81.3 & 75.1 & 78.1  \\
    \whline
    \end{tabular}
    
	\label{table:data}
	\vspace{-1.5mm}
\end{subtable}

==> tables/table3.tex <==
\def\x{{$\footnotesize \times$}}
\footnotesize
\begin{tabular}{l|c|c|c|c|c}
    \whline
	\multirow{2}*{Method} &\multirow{2}*{Ann} & \multirow{2}*{Pre}  &\multicolumn{3}{c}{CTW1500/\%}\cr\cline{4-6}  
	~ & ~ & ~ & P & R & F \cr\shline \hline
	\hline
	\textit{Strong Supervision} & ~ & ~ & ~ & ~ & ~  \\
    CTPN$^{\ast}$ & GT & - & 60.4 & 53.8 & 56.9  \\
    EAST$^{\ast}$ & GT & - & 78.7 & 49.1 & 60.4  \\
    SegLink$^{\ast}$ & GT & - & 42.3 & 40.0 & 40.8  \\
    PSENet~\cite{psenet} & GT & - & 80.6 & 75.6 & 78.0\\
    PSENet~\cite{psenet} & GT & \checkmark & 84.8 & 79.7 & 82.2 
    \\
    \hline\hline
    \textit{Weakly Supervision} & ~ & ~ & ~ & ~ & ~\\
    PSENet & b-GT & - &55.2 & 36.5 & 43.9  \\
    PSENet+PF & PL & \checkmark &78.8 & 76.3 & 77.5\textcolor[RGB]{96,177,87}{(+33.6)}  \\
    PSENet & b-GT & - & 58.5 & 40.2 & 47.6  \\
    PSENet+PF & PL &\checkmark & \textbf{82.4} & \textbf{80.6}&  \textbf{81.5}\textcolor[RGB]{96,177,87}{(+33.9)}  \\
     \whline
\end{tabular}


==> tables/table4.tex <==
\def\x{{$\footnotesize \times$}}
\footnotesize
\begin{tabular}{l|c|c|c|c|c}
    \whline
	\multirow{2}*{Method} &\multirow{2}*{Ann} & \multirow{2}*{Pre}  &\multicolumn{3}{c}{ICDAR2019-ArT/\%}\cr\cline{4-6}  
	~ & ~ & ~ & P & R & F \cr\shline \hline
	\hline
	\textit{Strong Supervision} & ~ & ~ & ~ & ~ & ~  \\
    TextRay~\cite{wang2020textray} $^{\ast}$ & GT & - & 75.8 & 58.6 & 66.1  \\
    PSENet$^{\dagger}$ & GT & - & 71.7 & 65.8 & 68.6\\
    PSENet$^{\dagger}$ & GT & \checkmark & 71.2 & 68.0 & 69.5
    \\
    \hline\hline
    \textit{Weakly Supervision} & ~ & ~ & ~ & ~ & ~\\
    PSENet & b-GT & - &49.0 & 41.4 & 44.9  \\
    PSENet+PF & PL & \checkmark &72.3 & 64.3 & 68.1\textcolor[RGB]{96,177,87}{(+23.2)}  \\
    PSENet & b-GT & - & 50.3 & 43.5 & 46.6  \\
    PSENet+PF & PL &\checkmark & \textbf{72.1} & \textbf{66.5} &  \textbf{69.2}\textcolor[RGB]{96,177,87}{(+22.6)}  \\
     \whline
\end{tabular}


==> tables/table7.tex <==
\begin{subtable}[t]{3.2in}
    \centering
	\setlength{\tabcolsep}{1.3mm}
	\small 
% 	\def\x{{$\footnotesize \times$}}
    \begin{tabular}{l|c|c|c|c}
    \whline
	\multirow{2}*{Method} & \multirow{2}*{Annotation}  &\multicolumn{3}{r}{Evaluation on Total-Text/\%}\cr\cline{3-5}  
	~ & ~ & Precision & Recall & F-score \cr\shline \hline
	\hline
    PSENet  & GT  & 80.4 & 76.5 & 78.4  \\
    PSENet & b-GT  & 46.5 & 43.6 & 45.0  \\
    PSENet  & PL(ST) & 80.3 & 73.5 & 76.8~(\textcolor[rgb]{0,0,1}{+31.8})   \\
    PSENet  & PL(Curved ST) & 81.7 & 75.6 & 78.5~(\textcolor[rgb]{0,0,1}{+33.5})  \\\shline \hline
    \multicolumn{5}{r}{Evaluation on MSRA-TD500/\%} \\\shline \hline
    PSENet  & GT  & 80.6 & 77.7 & 79.1  \\
    PSENet & b-GT  & 47.2 & 36.9 & 41.4  \\
    PSENet  & PL(ST) & 80.3 & 77.5 & 78.9~(\textcolor[rgb]{0,0,1}{+37.5}) \\\hline
    EAST  & GT  & 71.8 & 69.1 & 70.4  \\
    EAST$^*$  & PL(ST)  & 66.6 & 53.5 & 59.4  \\
    EAST & b-GT  & 40.5 & 31.1 & 35.2  \\
    EAST  & PL(ST) & 71.3 & 70.2 & 70.7~(\textcolor[rgb]{0,0,1}{+35.5})\\\whline
    \end{tabular}
	\label{table:Box}
	\vspace{5mm}
\end{subtable}
